Interoperability in the OpenDreamKit Project: The Math-in-the-Middle Approach

OpenDreamKit --- "Open Digital Research Environment Toolkit for the Advancement of Mathematics" --- is an H2020 EU Research Infrastructure project that aims at supporting, over the period 2015--2019, the ecosystem of open-source mathematical software systems. From that, OpenDreamKit will deliver a flexible toolkit enabling research groups to set up Virtual Research Environments, customised to meet the varied needs of research projects in pure mathematics and applications. An important step in the OpenDreamKit endeavor is to foster the interoperability between a variety of systems, ranging from computer algebra systems over mathematical databases to front-ends. This is the mission of the integration work package (WP6). We report on experiments and future plans with the \emph{Math-in-the-Middle} approach. This information architecture consists in a central mathematical ontology that documents the domain and fixes a joint vocabulary, combined with specifications of the functionalities of the various systems. Interaction between systems can then be enriched by pivoting off this information architecture.

==> examples/elliptic-curve.tex <==
\begin{mhmodnl}{elliptic-curve}{en}
  \begin{definition}[id=ec.q.def]
    An \defii{elliptic}{curve} over a \trefi[field]{field} $K$ is a smooth projective
    curve $E$ defined over $K$ of genus $1$ together with a (distinguished) $K$-rational 
    point $O$ (called the \defii{base}{point}) of $E$.
  \end{definition}
  
  \begin{assertion}[type=remark]
    The most commonly used model for \trefis{elliptic}{curve} is a plane cubic defined by
    a \trefi[Weierstrass-model]{Weierstrass}{equation}, with the \trefii{base}{point}
    being the unique point at infinity\ednote{reference}.
  \end{assertion}
  
  \begin{assertion}[type=remark]
    \guse{minimal-Weierstrass-model} Note that such an equation is not unique over
    $\RationalNumbers$. $E$ has a unique reduced
    \trefiii[minimal-Weierstrass-model]{minimal}{Weierstrass}{model}.
  \end{assertion}

  \begin{assertion}[id=ec.q.minimal-Weierstrass-model.def, 
    title=Minimal Weierstrass model of an elliptic curve on $\RationalNumbers$]
    Every \trefii[elliptic-curve]{elliptic}{curve} over $\RationalNumbers$ has an 
    integral Weierstrass model (or equation) of the form
    \[\minwe xy{\livar{a}1}{\livar{a}2}{\livar{a}3}{\livar{a}4}{\livar{a}6}\]
    where $\livar{a}1,\livar{a}2,\livar{a}3,\livar{a}4,\livar{a}6$ are integers.  Each
    such equation has a \trefi[discriminant-weierstrass-equation]{discriminant}
    $\wediscriminantOp$.
  \end{assertion}
\end{mhmodnl}

\begin{mhmodnl}{minimal-Weierstrass-model}{en}
    A \defi{minimal} \trefii{Weierstrass}{model} is one for which
    $\absolutevalue\wediscriminantOp$ is minimal among all Weierstrass models
    for the same curve.  For elliptic curves over $\RationalNumbers$, minimal 
    models exist, and there is a unique minimal model which satisfies the 
    additional constraints $\minset{\livar{a}1,\livar{a}3}{\set{0,1}}$, and 
    $\inset{\livar{a}2}{\set{-1,0,1}}$. 
    This is defined as the reduced minimal Weierstrass model of the elliptic curve.
  \end{definition}
\end{mhmodnl}


==> pgflibrarytikzmmt.code.tex <==
%

\def\outerthysep{.3mm}
\def\innerthysep{.5mm}
\tikzstyle{thy}=[draw,outer sep=\outerthysep,rounded corners,inner sep=\innerthysep]
\tikzstyle{primthy}=[thy,double]
\tikzstyle{thygraph}=[draw,outer sep=1mm,rounded corners,dashed]

\usetikzlibrary{arrows}
\newcommand{\@mmtarrowtip}{angle 45}
\newcommand{\@mmtreversearrowtip}{angle 45 reversed}
\newcommand{\@mmtarrowtipepi}{triangle 45}
\newcommand{\@mmtarrowtipmonoright}{right hook}
\newcommand{\@mmtarrowtipmonoleft}{left hook}
\newcommand{\@mmtarrowtippartial}{right to}
\newcommand{\@mmtarrowtippartialleft}{left to}
\newcommand{\@mmtreversearrowtippartial}{right to reversed}
\newcommand{\@mmtreversearrowtippartialleft}{left to reversed}

\usetikzlibrary{decorations,decorations.pathmorphing,decorations.markings}
\tikzstyle{morph}=[-\@mmtarrowtip,thick] 
\tikzstyle{mapsto}=[|-\@mmtarrowtip] %
\tikzstyle{struct}=[-\@mmtarrowtip,thick]
\tikzstyle{include}=[\@mmtarrowtipmonoright-\@mmtarrowtip,thick]
\tikzstyle{revinclude}=[\@mmtarrowtip-\@mmtarrowtipmonoright,thick]
\tikzstyle{pinclude}=[\@mmtarrowtipmonoright-\@mmtarrowtippartial,thick]
\tikzstyle{includeleft}=[\@mmtarrowtipmonoleft-\@mmtarrowtip,thick]
\tikzstyle{pincludeleft}=[\@mmtarrowtipmonoleft-\@mmtarrowtippartialleft,thick]
\tikzstyle{preview}=[decorate,
                                decoration={coil,aspect=0,amplitude=1pt,
                                                    segment length=6pt,
                                                    pre=lineto,pre length=3pt,
                                                    post=lineto,post length=5pt},
                                thick]
\tikzstyle{view}=[preview,-\@mmtarrowtip]
\tikzstyle{mview}=[preview,\@mmtarrowtipmonoright-\@mmtarrowtip]
\tikzstyle{pview}=[preview,-\@mmtarrowtippartial]
\tikzstyle{pmview}=[preview,\@mmtarrowtipmonoright-\@mmtarrowtippartial]
\tikzstyle{viewleft}=[preview,-\@mmtarrowtip]
\tikzstyle{mviewleft}=[preview,\@mmtarrowtipmonoleft-\@mmtarrowtip]
\tikzstyle{pviewleft}=[preview,-\@mmtarrowtippartialleft]
\tikzstyle{pmviewleft}=[preview,\@mmtarrowtipmonoleft-\@mmtarrowtippartialleft]
\tikzstyle{adoption}=[preview,thin,double,-\@mmtarrowtip]
\tikzstyle{biview}=[preview,\@mmtarrowtip-\@mmtarrowtip]
\tikzstyle{pbiview}=[preview,\@mmtreversearrowtippartial-\@mmtarrowtippartial]
\tikzstyle{pbiviewleft}=[preview,\@mmtreversearrowtippartialleft-\@mmtarrowtippartialleft]
\tikzstyle{defview}=[preview,densely dotted,-\@mmtarrowtip]
\tikzstyle{meta}=[dotted,-\@mmtarrowtip,thick]
\tikzstyle{conservative}=[hooks-\@mmtarrowtip,double] 
\tikzstyle{conservdev}=[hooks-\@mmtarrowtip,dashed,double] 

\tikzset{anti/.style={
    decoration={markings, mark=between positions 0.2 and 0.8 step 4mm with {
        \draw [thick,-] ++ (-3pt,-3pt) -- (3pt,3pt);}},
    postaction={decorate}}}

\tikzstyle{parallel}=[\@mmtarrowtip-\@mmtarrowtip,dashed]

\tikzstyle{prerealm}=[draw=blue!40,rectangle,rounded corners,inner sep=10pt,inner ysep=20pt]
\tikzstyle{realm}=[prerealm,fill=gray!4]
\tikzstyle{pillar}=[prerealm,fill=gray!10]

\newcommand\mmtthy[3]{\def\@second{#2}\def\@third{#3}%
\begin{array}{l}\textsf{#1}%
\ifx\@second\@empty\else\\\hline #2\fi%
\ifx\@third\@empty\else\\\hline #3\fi%
\end{array}}
\newcommand\mmtar[2][]{\raisebox{.5ex}{\tikz[#1]{\draw[#2] (0,0) -- (.6,0);}}}
\newcommand\nmmtar[3][]{\raisebox{.4ex}{\tikz[#1]{\draw[#2] (0,0) --
      node[above]{\ensuremath{\scriptstyle #3}} (.8,0);}}}
\usetikzlibrary{calc}
\newcommand\@pushout[4][]{\def\@test{#1}%
\ifx\@test\@empty\def\@@num{.5}\else\def\@@num{#1}\fi%
\begin{scope}[shift=($(#2)!\@@num!(#3)$)]\@nameuse{@#4pushoutsymb}\end{scope}} 
\newcommand\@nepushoutsymb{\draw +(-.2,0) -- +(0,0)  -- +(0,-.2);\fill +(-.1,-.1) circle (.03);}
\newcommand\nepushoutsymb{\tikz{\@nepushoutsymb}}
\newcommand\nepushout[3][]{\@pushout[#1]{#2}{#3}{ne}}

\newcommand\@sepushoutsymb{\draw +(-.2,0) -- +(0,0)  -- +(0,.2);\fill +(-.1,.1) circle (.03);}
\newcommand\sepushoutsymb{\tikz{\@sepushoutsymb}}
\newcommand\sepushout[3][]{\@pushout[#1]{#2}{#3}{se}}

\newcommand\@nwpushoutsymb{\draw +(.2,0) -- +(0,0)  -- +(0,-.2);\fill +(.1,-.1) circle (.03);}
\newcommand\nwpushoutsymb{\tikz{\@nwpushoutsymb}}
\newcommand\nwpushout[3][]{\@pushout[#1]{#2}{#3}{nw}}

\newcommand\@swpushoutsymb{\draw +(.2,0) -- +(0,0)  -- +(0,.2);\fill +(.1,.1) circle (.03);}
\newcommand\swpushoutsymb{\tikz{\@swpushoutsymb}}
\newcommand\swpushout[3][]{\@pushout[#1]{#2}{#3}{sw}}

\newcommand\@npushoutsymb{\draw +(-.1,-.1) -- +(0,0)  -- +(.1,-.1);\fill +(0,-.1) circle (.03);}
\newcommand\npushoutsymb{\tikz{\@npushoutsymb}}
\newcommand\npushout[3][]{\@pushout[#1]{#2}{#3}{n}}

\newcommand\@spushoutsymb{\draw +(-.1,.1) -- +(0,0)  -- +(.1,.1);\fill +(0,.1) circle (.03);}
\newcommand\spushoutsymb{\tikz{\@spushoutsymb}}
\newcommand\spushout[3][]{\@pushout[#1]{#2}{#3}{s}}

\newcommand\@wpushoutsymb{\draw +(-.1,-.1) -- +(0,0)  -- +(-.1,.1);\fill +(-.1,0) circle (.03);}
\newcommand\wpushoutsymb{\tikz{\@wpushoutsymb}}
\newcommand\wpushout[3][]{\@pushout[#1]{#2}{#3}{w}}

\newcommand\@epushoutsymb{\draw +(.1,.1) -- +(0,0)  -- +(.1,-.1);\fill +(.1,0) circle (.03);}
\newcommand\epushoutsymb{\tikz{\@epushoutsymb}}
\newcommand\epushout[3][]{\@pushout[#1]{#2}{#3}{e}}




==> tikz/localpaths.tex <==
% this file defines root path local repository
\defpath{MathHub}{/Users/kohlhase/localmh/MathHub}
\mhcurrentrepos{MiKoMH/talks}
\libinput{WApersons}
% we also set the base URI for the LaTeXML transformation
\baseURI[\MathHub{}]{https://mathhub.info/MiKoMH/talks}


==> tikzlibrarymmt.code.tex <==
\input{pgflibrarytikzmmt.code.tex}


